On Extracting Data from Tables that are Encoded using HTML

Tables are a common means to display data in human-friendly formats. Many authors have worked on proposals to extract those data back since this has many interesting applications. In this article, we summarise and compare many of the proposals to extract data from tables that are encoded using HTML and have been published between $2000$ and $2018$. We first present a vocabulary that homogenises the terminology used in this field; next, we use it to summarise the proposals; finally, we compare them side by side. Our analysis highlights several challenges to which no proposal provides a conclusive solution and a few more that have not been addressed sufficiently; simply put, no proposal provides a complete solution to the problem, which seems to suggest that this research field shall keep active in the near future. We have also realised that there is no consensus regarding the datasets and the methods used to evaluate the proposals, which hampers comparing the experimental results.

==> Dirty-Tricks.tex <==
% Dirty-Tricks.tex

\makeatletter

     % Some math fixes

    \let\save@pfun=\pfun
    \def\pfun{\mathrel{\save@pfun}}

    % URL styles

    \urlstyle{sf}

    % This typesets \parapraphs in bold face and underlined.

    \let\save@paragraph=\paragraph
    \def\paragraph#1{\vspace{3pt plus 1pt minus 1pt}\noindent{\bfseries #1:\space}\ignorespaces}

    % Some small changes to common environments

    \let\save@enddefinition=\enddefinition
    \def\enddefinition{\hfill$\square$}

    % Some small changes to floats

    \def\floathook{\centering\scriptsize}

    \let\savefigure=\figure
    \def\figure{\savefigure\floathook}

    \let\savetable=\table
    \def\table{\savetable\floathook}

    \renewenvironment{figure*}{\@dblfloat{figure}[!htbp]\floathook}{\end@dblfloat}
    \renewenvironment{table*}{\@dblfloat{table}\floathook}{\end@dblfloat}

    % This helps LaTeX place floats a lot better.

    \def\fps@figure{tb!}
    \def\fps@table{tb!}
    \renewcommand\ps@empty{\ps@plain}

    \setcounter{topnumber}{2}
    \setcounter{bottomnumber}{1}
    \setcounter{totalnumber}{2}
    \setcounter{dbltopnumber}{2}

    \renewcommand\topfraction{1.00}
    \renewcommand\bottomfraction{1.00}
    \renewcommand\dbltopfraction{1.00}

    \renewcommand\textfraction{0.00}
    \renewcommand\floatpagefraction{1.00}
    \renewcommand\dblfloatpagefraction{1.00}

    % Title

    \let\save@title=\title
    \def\title#1{\save@title{\bfseries #1}}

    % This should force LaTeX to flush every page at its bottom

    \flushbottom

    % Make comma discretionary in math mode

    \def\old@comma{,}
    \catcode`\,=13
    \def,{%
        \ifmmode%
            \old@comma\discretionary{}{}{}%
        \else%
            \old@comma%
        \fi%
    }

\makeatother 

==> src/Biographies.tex <==
% Biographies.tex

\bigbreak

\begin{bio}{picture-roldan}{Juan C. Roldán}
is working as a researcher for the University of Seville.  His research focuses on large-scale web data extraction, with an emphasis on extracting data from HTML tables as a means to feed Data Science applications.
\end{bio}

\begin{bio}{picture-jimenez}{Patricia Jiménez}
is working as a lecturer for the University of Seville.  Her research focuses on large-scale web data extraction, with an emphasis on methods to evaluate their performance regarding both efficiency and effectiveness.
\end{bio}

\begin{bio}{picture-corchuelo}{Rafael Corchuelo}
is working as a reader for the University of Seville. His research focuses on application and information integration, with an emphasis on web information extraction and social media analytics.
\end{bio}

